Analysis of Ward's Method

We study Ward's method for the hierarchical $k$-means problem. This popular greedy heuristic is based on the \emph{complete linkage} paradigm: Starting with all data points as singleton clusters, it successively merges two clusters to form a clustering with one cluster less. The pair of clusters is chosen to (locally) minimize the $k$-means cost of the clustering in the next step. Complete linkage algorithms are very popular for hierarchical clustering problems, yet their theoretical properties have been studied relatively little. For the Euclidean $k$-center problem, Ackermann et al. show that the $k$-clustering in the hierarchy computed by complete linkage has a worst-case approximation ratio of $\Theta(\log k)$. If the data lies in $\mathbb{R}^d$ for constant dimension $d$, the guarantee improves to $\mathcal{O}(1)$, but the $\mathcal{O}$-notation hides a linear dependence on $d$. Complete linkage for $k$-median or $k$-means has not been analyzed so far. In this paper, we show that Ward's method computes a $2$-approximation with respect to the $k$-means objective function if the optimal $k$-clustering is well separated. If additionally the optimal clustering also satisfies a balance condition, then Ward's method fully recovers the optimum solution. These results hold in arbitrary dimension. We accompany our positive results with a lower bound of $\Omega((3/2)^d)$ for data sets in $\mathbb{R}^d$ that holds if no separation is guaranteed, and with lower bounds when the guaranteed separation is not sufficiently strong. Finally, we show that Ward produces an $\mathcal{O}(1)$-approximative clustering for one-dimensional data sets.

==> input_example_nonmonotone.tex <==
\begin{figure}
\centering
\begin{tikzpicture}

\node [draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (a) at (0:1cm) {};
\node [draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (b) at (120:1cm) {};
\node [draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (c) at (240:1cm) {};

\draw (a) to node {} (b);
\draw (b) to node {} (c);
\draw (a) to node {} (c);

\begin{scope}[xshift=5cm]
\node [label=right:{$2$},draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (a) at (0:1cm) {};
\node [label=above:{$2$},draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (b) at (120:1cm) {};
\node [label=below:{$2$},draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (c) at (240:1cm) {};

\node [label=above:{$1$},draw,fill,circle,inner sep=0cm,minimum width=0.1cm] (o) at (0,0) {};

\draw (a) to node {} (o);
\draw (b) to node {} (o);
\draw (c) to node {} (o);
\end{scope}
\end{tikzpicture}
\caption{Two examples for the non-monotonicity of the greedy algorithm for $k$-median.\label{fig:discretenotmonotone}}
\end{figure}

\section{Greedy is not monotone for \texorpdfstring{$k$}{k}-median}\label{sec:kmediannotmonotone}
Figure~\ref{fig:discretenotmonotone} consists of two examples showing that the greedy method that works like Ward, but for $k$-median clustering, is not monotone. On the left, we see an example for the Euclidean $k$-median problem. It is simply an isosceles triangle; say that the distance between any two points is $1$. The $3$-clustering is free. The first merge costs $1$, no matter which two points are merged. For the resulting cluster, any point on the line between the two points is an optimal center. In particular, when merging with the third point, choosing the mid point between the first two points still results in a cost of $1$ for these two points; but the distance of this point to the third is only $\sqrt{3}/2$. Thus, the second merge is cheaper than the first (it is indeed even slightly cheaper than $\sqrt{3}/2$ because the optimal center of the $1$-clustering does not lie on the line between the first two points). 

We can construct a similar example for $k$-median in finite discrete space. Here, the input points come with a finite metric, and the centers can only be chosen from the input points. Consider the right side of Figure~\ref{fig:discretenotmonotone}. There are four points, out of which three have weight $2$. The edges have unit length and all other distances are shortest paths in the graph. The first merge has minimal cost if one of the outer points is merged with the point in the middle. This results in a cost of $1$ if the center is placed on the outer point. The second merge has to be with a different outer point, or the two outer points are merged. In both cases, the merge costs $4$, and the final merge costs $2$, i.e., violates monotonicity.
